SU(3) Approach to Hypernuclear Interactions and Spectroscopy

The $SU(3)$ meson exchange approach to interactions within the baryon octet and nuclear density functional theory are used to derive an \emph{ab initio} description of hypernuclear interactions. The density dependence of interactions is recast into a DFT with density dependent interaction vertices. The field-theoretical structure is retained by expressing the vertices as functionals of the matter field operators. Applications to infinite hypermatter and neutron star matter are discussed. A new approach is presented allowing to determine in-medium coupling constants out of the $NN$-vertex functionals, obtained e.g. by DBHF theory, for the full baryon octet by exploiting $SU(3)$ relations.

==> OBE_v3.tex <==
\section{Interactions in the baryon octet}\label{sec:OctetInter}

The statement that the quantitative understanding of hypernuclei requires an accurate knowledge of hyperon-hyperon $(YY)$ and hyperon-nucleon $(YN)$ interactions sounds obvious but, in fact, is far from being trivial. The solution of this basic task is still far from being under control to a satisfactory level at the degree of accuracy required for a hypernuclear theory of predictive power. The progress made in the last decade or so for $S=-1$ systems is only part of the full story since this involves mainly single-$\Lambda$ hypernuclei, supplementing the few data points from old $p\Lambda$ and $p\Sigma$ experiments, e.g. in \cite{Ale:1968,Sec:1968,Eis:1971}. The latter are essential input for the approaches developed over the years by several groups. While the Nijmegen \cite{Nijmegen,Yama:2014} and the Juelich group \cite{Juelich}, respectively, are using a baryon-meson approach, the Kyoto-Niigata group \cite{Niigata} favors a quark-meson picture, finally ending also in meson-exchange interactions. However, none of the existing parameter sets is in any sense constrained with respect to interactions in the $|S|\geq 2$ channels. As a consequence, the implementation of SU(3) flavor symmetry is incomplete. In view of this situation, we found it necessary to reconsider interactions in the lowest SU(3) baryon octet with special emphasis on in-medium interactions. As a long-term program the approach will allow to test interactions more directly under the dynamical conditions of strangeness and hypernuclear production reactions with leptonic, hadronic, and nuclear probes, up to heavy ion reactions at relativistic energies. Hyperon and hypernuclear data from reactions are providing a wealth of information which has not yet been taken advantage of in full breadth.

We introduce the flavour spinor $\Psi_F$
\beq
\Psi_F = \left( \Psi_N, \Psi_\Lambda, \Psi_\Sigma, \Psi_\Xi \right)^{\text{T}}
\label{eq:FlavorSp}
\eeq
being composed of the isospin multiplets
\beq
\Psi_N = \left( \begin{array}{c} \psi_p \\ \psi_n \end{array} \right),\quad
\Psi_\Lambda = \psi_\Lambda,\quad
\Psi_\Sigma = \left( \begin{array}{c}
\psi_{\Sigma^+} \\ \psi_{\Sigma^0} \\ \psi_{\Sigma^-} \end{array} \right),\quad
\Psi_\Xi = \left( \begin{array}{c}
\psi_{\Xi^0} \\ \psi_{\Xi^-} \end{array} \right)
\eeq
where $\psi_i$ are Dirac spinors. The full Lagrangian is structured in an
isospin symmetric way. The mesonic sector includes the pseudo-scalar, vector, and scalar nonets. Of special interest for nuclear matter and nuclear structure research are the mean-field producing meson fields, involving isoscalar-scalar mesons $\sigma$, $\sigma_s$, the isovector-scalar $\delta=a_0(980)$ meson, and their isoscalar-vector counterparts $\omega,\phi$ and the isovector-vector $\rho$ meson, respectively. For finite nuclei, the photon field $A^\mu_\gamma$ is included. Thus, we are dealing with the Lagrangian
\be\label{Lagrangian}
\Lcal = \Lcal_{B} + \Lcal_{M} + \Lcal_{int}
\ee
accounting for the free motion of baryons with mass matrix $\hat{M}$,
\be
\Lcal_{B} = \Psib_{F} \left[ i\gamma_\mu\p^\mu
                              - \hat{M} \right] \Psi_{F} \quad ,
\ee
and the Lagrangian density of massive mesons,
\be
\Lcal_{M} =\frac{1}{2} \sum_{i = P,S,V}
\left(\p_\mu\Phi_i\p^\mu\Phi_i - m_{\Phi_i}^2\Phi_i^2\right)
           - \frac{1}{2} \sum_{\kappa = V}
             \left( \frac{1}{2} F^{(\kappa)^2} - m_\kappa^2 A^{(\kappa)^2}
\right)
\ee
where $P,S,V$ denote summations over the lowest nonet pseudo-scalar, scalar, and vector mesons, the latter including also the photon. The field strength tensor of the vector mesons is given by
\beq
F^{(\kappa)}_{\mu\nu} = \p_\mu A_\nu^{(\kappa)} - \p_\nu A_\mu^{(\kappa)} \quad .
\label{eq:Fmunu}
\eeq
Baryon-meson interactions, contained in $\Lcal_{int}$, are specified below.

SU(3) octet physics is based on treating the eight baryons on equal footing. Although SU(3) flavor symmetry is broken by about 20\% on the mass scale, it is still meaningful to exploit the relations among coupling constants, thus defining a guideline and reducing the number of free parameters considerably. The eight $J^P={\textstyle\frac{1}{2}}^+$ baryons are collected into a traceless matrix $B$, which is given by a superposition of the eight Gell-Mann matrices $\lambda_i$, leading to the familiar form
\begin{equation}
  B = \left( \begin{array}{ccc}
      {\displaystyle\frac{\Sigma^{0}}{\sqrt{2}}+\frac{\Lambda}{\sqrt{6}}}
               &  \Sigma^{+}  &  p  \\[2mm]
      \Sigma^{-} & {\displaystyle-\frac{\Sigma^{0}}{\sqrt{2}}
                   +\frac{\Lambda}{\sqrt{6}}}  &  n \\[2mm]
      -\Xi^{-} & \Xi^{0} &  {\displaystyle-\frac{2\Lambda}{\sqrt{6}}}
             \end{array} \right),
\end{equation}
and which is invariant under SU(3) transformations. The pseudo-scalar($Ps$), vector ($V$), and, last but not least, the scalar ($S$)  meson nonets are expressed correspondingly. Taking the pseudo-scalar mesons with $J^P=0^-$ as an example we obtain the octet matrix $P_{8}$
\begin{equation}
   P_{8} = \left( \begin{array}{ccc}
      {\displaystyle\frac{\pi^{0}}{\sqrt{2}}+\frac{\eta_{8}}{\sqrt{6}}}
             & \pi^{+}  &  K^{+}  \\[2mm]
      \pi^{-} & {\displaystyle-\frac{\pi^{0}}{\sqrt{2}}
         +\frac{\eta_{8}}{\sqrt{6}}}  &   K^{0} \\[2mm]
      K^{-}  &  \overline{{K}^{0}}
             &  {\displaystyle-\frac{2\eta_{8}}{\sqrt{6}}}
             \end{array} \right).
\end{equation}
which, for the full nonet, has to be completed by the singlet matrix $P_1$, given by the unit matrix multiplied by $\eta_0/\sqrt{3}$. We define the SU(3)-invariant combinations
\begin{eqnarray}
  \left[\overline{B}BP_8\right]_{F} &=& {\rm Tr}\left(\left[\overline{B},B\right]_{-}P_{8}\right)\quad , \quad
  \left[\overline{B}BP_8\right]_{D}
= {\rm Tr}\left(\left[\overline{B},B\right]_{+}P_{8}\right)\quad , \nonumber \\
\left[\overline{B}BP_0\right]_{S} &=& {\rm Tr}(\overline{B}B){\rm Tr}(P_{0})
\end{eqnarray}
where $F$ and $D$  correspond to anti-symmetric and symmetric combinations of field operators, as indicated by the commutators and anti-commutators, $[A,B]_\mp$, respectively. With these relations we obtain the interaction Lagrangian
\begin{equation}
   {\cal L}_{I} =  - \left\{
     g_F\left[\overline{B}BP_8\right]_{F}  +
     g_D\left[\overline{B}BP_8\right]_{D}\right\}\, - \,
     g_S\left[\overline{B}BP_0\right]_{S},             \label{eq:LIsu3}
\end{equation}
with the generic SU(3) coupling constants $\{g_{D,F,S}\}_P$. Corresponding structures with their own sets $\{g_{D,F,S}\}_{S,V}$ exist for the scalar and vector multiplets.  The square-root factors are introduced following a commonly used convention. We introduce the isospin doublets
\begin{equation}
  N=\left(\begin{array}{c} p \\ n \end{array} \right), \ \ \
  \Xi=\left(\begin{array}{c} \Xi^{0} \\ \Xi^{-} \end{array} \right), \ \ \
  K=\left(\begin{array}{c} K^{+} \\ K^{0} \end{array} \right),
  \ \ \   K_{c}=\left(\begin{array}{c} \overline{K^{0}} \\
               -K^{-} \end{array} \right) \quad .        \label{eq:doublets}
\end{equation}
The $\Sigma$ hyperon and the pion isovector-triplets are expressed in the basis defined by the spherical unit vectors $\bm{e}_{\pm,0}$ which leads to
\begin{equation}
  \bm{\Sigma}\!\cdot\!\bm{\pi} = \Sigma^{+}\pi^{-}+\Sigma^{0}\pi^{0}+\Sigma^{-}\pi^{+} \quad ,
\end{equation}
also serving to fix phases. We define the pseudo-vector Dirac-vertex operator $\Gamma=\gamma_{5}\gamma_{\mu}\partial^{\mu}$. By evaluating the $F$- and $D$-type couplings, Eq.~(\ref{eq:LIsu3}), we obtain the pseudo-scalar octet-meson interaction Lagrangian
\begin{eqnarray}
  &&m_{\pi}{\cal L}_{8} \sim \nonumber \\
  &-&g_{N\!\pi}(\overline{N}\Gamma\bm{\tau}N)\!\cdot\!\bm{\pi}
  +ig_{\Sigma\Sigma\pi}(\overline{\bm{\Sigma}}\!\times\!\Gamma\bm{\Sigma})
      \!\cdot\!\bm{\pi}\nonumber \\
  &-&g_{\Lambda\Sigma\pi}(\overline{\Lambda}\Gamma\bm{\Sigma}+
      \overline{\bm{\Sigma}}\Gamma\Lambda)\!\cdot\!\bm{\pi}
  -g_{\Xi\Xi\pi}(\overline{\Xi}\Gamma\bm{\tau}\Xi)\!\cdot\!\bm{\pi}
            \nonumber\\
 &-&g_{\Lambda N\!K}\left[(\overline{N}\Gamma K)\Lambda
         +\overline{\Lambda}\Gamma(\overline{K}N)\right]
   -g_{\Xi\Lambda K}\left[(\overline{\Xi}\Gamma K_{c})\Lambda
         +\overline{\Lambda}\Gamma (\overline{K_{c}}\Xi)\right] \nonumber\\
 &-&g_{\Sigma N\!K}\left[\overline{\bm{\Sigma}}\!\cdot\Gamma\!
         (\overline{K}\bm{\tau}N)+(\overline{N}\Gamma\bm{\tau}K)
         \!\cdot\!\bm{\Sigma}\right]
   -g_{\Xi\Sigma K}\left[\overline{\bm{\Sigma}}\!\cdot\!
       \Gamma (\overline{K_{c}}\bm{\tau}\Xi)
     +(\overline{\Xi}\Gamma\bm{\tau}K_{c})\!\cdot\!\bm{\Sigma}\right]
                                         \nonumber\\
 &-&g_{N\!N\eta_{8}}(\overline{N}\Gamma N)\eta_{8}
   -g_{\Lambda\Lambda\eta_{8}}(\overline{\Lambda}\Gamma\Lambda)\eta_{8}
   -g_{\Sigma\Sigma\eta_{8}}(\overline{\bm{\Sigma}}\!\cdot\!\Gamma
       \bm{\Sigma})\eta_{8}
   -g_{\Xi\Xi\eta_{8}}(\overline{\Xi}\Gamma\Xi)\eta_{8}.    \label{eq:Lbar8}
\end{eqnarray}
where the charged-pion mass serves as the mass-scale compensating the effect of the derivative coupling.
The - in total 16 - pseudo-scalar $BB'$-meson vertices are completely fixed by the three nonet coupling constants $(f_8,f_1,\alpha)$ or, likewise, by $(g_{D},g_{F},g_S)_P$. Corresponding relations are valid also for the vector and the scalar nonets, $V^\mu$ and $S$, with coupling constants $(g_{D},g_{F},g_{S})_{S,V}$, respectively. \footnote{We neglect the rank-2 tensor $BB'$-vector meson coupling}.

The coupling constants of the three nonets, ($m=P,V,S$), obey a common structure. Denoting the isoscalar octet meson by $f\in \{\eta_8,\omega_8,\sigma_8 \}$, the isovector octet meson by $a\in \{\pi,\rho,\delta \}$, and the isospin doublet meson by $K\in \{K^{0,-},K^{*0-},K^*_s \}$, the interaction strengths are determined by the relations
\begin{equation}
  \begin{array}{lll}
   g_{N\!N a}               = \sqrt{2}(g_{D}+g_{F}),                               \ \ \  &
   g_{\Lambda N\!K}          =-\frac{\sqrt{2}}{\sqrt{3}}(g_{D}+2g_{F}),\ \ \  &
   g_{N\!Nf}          = \frac{1}{2}(3g_{F}-g_{D}),
      \\
   g_{\Sigma\Sigma a}       = \sqrt{2}g_{F},                        \ \ \  &
   g_{\Xi\Lambda K}          = \frac{\sqrt{2}}{\sqrt{3}}(3g_{F}-g_{D}),\ \ \  &
   g_{\Lambda\Lambda f} =-\frac{\sqrt{2}}{\sqrt{3}}g_{D},
      \\
   g_{\Lambda\Sigma a}      = \frac{\sqrt{2}}{\sqrt{3}}g_{D}, \ \ \  &
   g_{\Sigma N\!K}           = \sqrt{2}(g_{D}-g_{F}),                    \ \ \  &
   g_{\Sigma\Sigma f}  = \frac{\sqrt{2}}{\sqrt{3}}g_{D},
      \\
   g_{\Xi\Xi a}             =-\sqrt{2}(g_{D}-g_{F}),                    \ \ \  &
   g_{\Xi\Sigma K}           =-2(g_{D}+g_{F}),                               \ \ \  &
   g_{\Xi\Xi f}        =-\frac{\sqrt{2}}{\sqrt{3}}(3g_{F}+g_{D}).
  \end{array}
                        \label{eq:goct}
\end{equation}
where $g_{D,F,S}$ denotes either set of pseudo-scalar, vector, and scalar cuplings. The interactions due to exchange of the isoscalar-singlet meson $f'\in \{\eta_1,\omega_1,\sigma_1 \}$  are treated accordingly with the result
\begin{equation}
   g_{N\!N f'}=g_{\Lambda\Lambda f'} =g_{\Sigma\Sigma f'}=g_{\Xi\Xi f'} = g_{S}.  \label{eq:gsin}
\end{equation}

\subsection{Dynamical SU(3) symmetry breaking}\label{ssec:SymBreak}
From the above relations, the advantage of referring to SU(3) symmetry is obvious: For each type of meson (pseudo-scalar, vector, scalar) only four independent parameters are required to characterize their interaction strengths with all possible baryons. These are the singlet
coupling constant $g_S$, the octet coupling constants $g_D,g_F$, and eventually the three mixing angles $\theta_{P,V,S}$, one for each meson multiplet, which relate the physical, dressed isoscalar mesons to their bare octet and singlet counterparts. Likewise, a different set of parameters is used frequently to describe the $(P,V,S)$ multiplets, given by $f_8=g_D+g_F$, the ratios $\alpha_8=g_F/(g_F+g_D)$, and the singlet coupling constant $f_1=g_S$. It should also be noted that representations are in use extracting factors $\sqrt{2}$ and $\frac{}{\sqrt{3}}$ from the ($D,F$)-type and the $S$-type Lagrangians, respectively.

SU(3) symmetry, however, is broken at several levels and SU(3) relations will not be satisfied exactly. An obvious one is the non-degeneracy of the physical baryon and meson masses within the multiplets. As discussed below, this splitting leads to additional complex structure in the set of coupled equations for the scattering amplitudes because the various baryon-baryon ($BB'$) channels open at different threshold energies $\sqrt{s_{BB'}}=m_B+m_{B'}$. At energies $s<s_{BB'}$ a given $BB'$-channel does not contain asymptotic flux but contributes as a virtual state. Thus, $N\Lambda$ scattering, for example, will be modified at any energy by admixtures of $N\Sigma$ channels.

In addition, SU(3) symmetry is broken explicitly by the fact that $\Lambda$ and $\Sigma^0$ have the same quark content but coupled to different total isospin. There is an appreciable electro-weak mixing between the ideal isospin-pure $\Lambda$ and $\Sigma^0$ states~\cite{Dal64}. Exact SU(3) symmetry of strong interactions predicts $f_{\Lambda\Lambda\pi^0}=0$, but $\Lambda$-$\Sigma^0$ mixing results in a weak, but non-zero $\Lambda\Lambda\pi$ coupling constant for the physical $\Lambda$-hyperon, as derived by Dalitz and von Hippel~\cite{Dal64} already in the early days of strangeness physics,
\begin{equation}
  g_{\Lambda\Lambda\pi}=-2\frac{\langle\Sigma^0|\delta M|\Lambda\rangle}
             {M_{\Sigma^0}-M_{\Lambda}}\,f_{\Lambda\Sigma\pi},
\end{equation}
where the $\Sigma\Lambda$ element of the mass matrix is given by
\begin{equation}
   \langle\Sigma^0|\delta M|\Lambda\rangle=
       \left[M_{\Sigma^0}-M_{\Sigma^+}+M_p-M_n\right]/\sqrt{3}.
\end{equation}
Substituting for the physical baryon masses, we find
$ g_{\Lambda\Lambda\pi}=c_b\,f_{\Lambda\Sigma\pi}$ where $c_b=-0.0283...$ is the symmetry breaking coefficient. From the nucleon-nucleon-pion part of the interaction Lagrangian, Eq. \ref{eq:Lbar8}, we find
\begin{equation}
    (\overline{N}\bm{\tau}N)\!\cdot\!\bm{\pi} =
    \overline{p}p\pi^0-\overline{n}n\pi^0+\sqrt{2}\,\overline{p}n\pi^+
                      +\sqrt{2}\,\overline{n}p\pi^-,
\end{equation}
and the neutral pion is seen to couple with opposite sign to neutrons and protons. This implies that the non-zero $f_{\Lambda\Lambda\pi^0}$ coupling produces considerable deviations from charge symmetry in $\Lambda p$ and $\Lambda n$ interactions. Obviously, $\Lambda$-$\Sigma^0$ mixing also gives rise to non-zero $\Lambda\Lambda$ coupling constants for any (neutral) isovector meson, in particular for the $\rho$ vector meson and the $\delta/a_0(980)$, the isovector member of the $0^+$ meson octet, respectively but the latter couplings give rise to much smaller effects.

As seen from Eq.(\ref{eq:goct}), $\Lambda$ and $\Sigma$ hyperons are coupled by strong interactions leading to a strangeness- and isospin/charge-conserving dynamical mixing of $N\Lambda$ and $N\Sigma$ channels. Again, corresponding effects are present also for vector-isovector and scalar-isovector mesons. As a result, channels of the same total strangeness $S$ and fixed total charge $Q$ are coupled already on the level of the elementary vertices in free space. In asymmetric nuclear matter, this effect is enhanced through the isovector mean-field produced by the $\rho_0$ and the $\delta_0$ meson fields. This leads to a density dependent $\Lambda\Sigma^0$ mixing being proportional to the isovector mean-field $U_1\sim \rho_1$ and determined by the isovector baryon density $\rho_1=\rho_n-\rho_p$ plus possible contributions from charged hyperons. As a result, $\Lambda$ and $\Sigma^0$ become quasi-particles with mass eigenstates different from the flavor eigenstates. The total isospin is of course conserved by virtue of the background medium.

\section{Interactions in Free Space}\label{sec:FreeSpace}
On the tree-level the octet interaction Lagrangians discussed in the previous section correspond to standard One Boson Exchange ($OBE$) amplitudes. The full interaction amplitudes require the solution of the Bethe-Salpeter equation. As in \cite{Machleidt:1989,Dejong:1998}, we reduce the problem to an effective Lippmann-Schwinger equation by projecting out the time-like components by the Thompson method. However, different from the better known SU(2) nucleon-nucleon case \cite{Machleidt:1989,Dejong:1998}, the full SU(3) problem leads to a set of coupled equations describing interactions within the set of channels of fixed strangeness $S=0,-1\cdots -4$ and total charge $Q$, respectively, where the latter corresponds to fix the third component of the total isospin.

\textbf{MADHUMITA: PLEASE DISCUSS HERE THE MULITPLETS FOR FIXED S AND CHARGE Q (TABLE!) AND ALSO ADD AND DISCUSS THE FIGURE WITH THE KINEMATICAL THRESHOLDS.}

Hence, in momentum representation and after performing a partial wave decomposition we have to solve the coupled integral equation
\be\label{eq:Tmat}
T_{ab}(q,q')=\tilde{V}_{ab}(q,q')+\sum_c{\frac{1}{2\pi^2}\int{dkk^2V_{ac}(q,k)Q^{(c)}_F(k,s)G_c(k,s)T_{cb}(k,q') } }
\ee
where the indices $a,b,c$ account for all relevant quantum numbers in the corresponding flavor and partial wave channels, thus including a summation over the set of coupled baryon channels. $G_c$ denotes Green's function in the intermediate channel $c$, to be evaluated at the on-shell total center-of-mass energy, fixed by the Mandelstam variable $s$. In nuclear matter, the Pauli-projector
\be
Q^{(c)}_F=\Theta(k^2_1-k^2_{F1})\Theta(k^2_2-k^2_{F2})
\ee
accounts by the step-functions for the Pauli-principle by blocking the occupied states inside the Fermi spheres $k_{F1,2}$ of particle 1 and particle 2. In practice, we use  angle-averaged Pauli-projectors. In free space we have $Q^{(c)}_F\equiv 1$. Additional in-medium modifications are introduced by self-energy, mainly modifying the propagators. In-medium interactions will be discussed in more detail in later sections. In free-space, $Q_F$ reduces of course to the unit operator.

The Born-term contributes only at energies above the kinematical thresholds $s_{thr}=s_a,s_b$
\be
\tilde{V}(q,q')=V(q,q')\Theta(s-s_{a})\Theta(s-s_{b})
\ee
thus accounting explicitly for SU(3) mass symmetry breaking. By a properly chosen quadrature method Eq.(\ref{eq:Tmat}) is conveniently transformed into a numerically easy to solve linear system, see e.g. \cite{Machleidt:1989}. The $BB'$ scattering matrix elements are determined numerically in by expressing the T.matrix in terms of the K-matrix, $T=\left(1-iK  \right){-1}K$ which is standard technique in reaction theory \cite{Machleidt:1989}. The K-matrix obeys a system  of as in Eq. \ref{eq:Tmat} but using only the Cauchy Principal Value part of the intermediate propagators. Thus, the numerical problem reduces to the solution of a linear system of equations with real coefficients. The bare coupling constants $\left\{g_{S,D,F}\right\}_{P,S,V}$ are determined phenomenologically by fit to data. At present, the scarce data base, however, puts severe constraints on the precision of the derived values.

For a process $B_1+B_2\to B_3+B_4$, the latter are Lorentz-invariants of vertex functionals and meson propagators,
\beq\label{obe}
V^{BB'}_{\alpha}(q',q)=g_{B_1B_3\alpha} \rho_{B_1B_3\alpha}(q,q')) D_\alpha(Q)
 \rho^\alpha_{B_2B_4}(-q,-q'))g_{B_2B_4\alpha}
\eeq
where in- and out-states are denotes by $B$ and $B'$, respectively. We have introduced the density matrices
\be
\rho_{BB'\alpha}(k,k'))=\bar{u}^{B}(k')\kappa_\alpha u^{B'}(k) \quad .
\ee
The meson propagators $D_\alpha$ depend on the 4-momentum transfer $Q$ which is either in the $t=(k'-k)^2$ or the $u=(k+k')^2$ channel, respectively. In the two-body center-of-momentum frame, the 4-momenta in the in- and outgoing channels $(B_1,$ $B'_2)$ and $(B_3,$
$B'_4)$, respectively, are $k,k'$ with $k=(\omega,\bm(k))$. On the mass-shell, $k^2=q^2=m^2_B$ and the space-like components $\bm{q}$ are given by the total Mandelstam-energy $s_{12}=(p_1+p_2)^2$,
\be
q^2=\frac{1}{4s_{12}}\left( s_{12}+(M_1+M_2)^2 \right)\left( s_{12}+(M_1-M_2)^2 \right)\\
\ee
and $\bm{q}'$ is fixed accordingly. Dirac spinors are indicated by $u^B(k)$. $\kappa_\alpha$ indicates the Dirac and flavour structure of the vertex with the previously introduced bare coupling constants $g_{BB\alpha}$ and $g_{B'B'\alpha}$, contracted over Dirac and flavour indices as
indicated by $\kappa_\alpha \cdot \kappa^\alpha$.

The tree-level matrix elements $V_{BB'}=\sum_\alpha{V_{BB'\alpha}}$ are entering as kernels into the Bethe-Salpeter equation. The latter is solved in three-dimensional reduction, resulting in an equivalent effective Lippmann-Schwinger equation for the K- or R-matrix, see e.g. \cite{Dejong:1998},
\bea\label{eq:BbS}
&&R^{BB'}(q',q)=V_{BB'}(q',q)\nonumber \\ &+&
\sum_{B''}{P\int{\frac{d^3k}{(2\pi)^3}~V_{BB''}(q',k)G_{B''}(k,\sqrt{s})\bar{Q}_F(k,\sqrt{s},k_{FB''})R_{B''B'}(k,q)}}\quad .
\eea
which accounts for the ladder-resummation of two-body interactions in free space and infinite nuclear matter. The integration is treated as a Cauchy-Principal Value integral, as indicated. Since in free space $Q_F$ reduces to the unity operator. The reduction to an equivalent Lippmann-Schwinger eqaution in three dimensions is performed in the Blankenbecler-Sugar scheme. The two-particle propagator becomes in Blankenbecler-Sugar representation,
\be\label{eq:GBbS}
G_{bBS}(k,\sqrt{s})=4\sqrt{\frac{M_1M_2}{E_1(k)E_2(k)}}\frac{1}{(E_1(k)+E_2(k))^2-s} \quad ,
\ee
to be used for positive energy states only. Hence, in free space $R$ reduces to the usual $K$-matrix from which phase shifts and scattering amplitudes are calculated.

\textbf{MADHUMITA: DISCUSS CROSS SECTIONS AND THE FIT, ADD A TABLE WITH THE COUPLING CONSTANTS, TRY TO DETERMINE THE CORRESPONDING $g_{D,F,S}$ COUPLINGS}


\section{Baryon-Baryon Interactions in Infinite Nuclear Matter}\label{sec:BB_Infinite}

The extension to in-medium scattering is readily achieved on the basis of the T-matrix, Eq. \ref{eq:Tmat}. In a medium, an important role is played by the Pauli-projector $Q_F$.  The Pauli-projector is given in terms of the 3-momenta $k_{i}$ in the nuclear matter frame and the Fermi-momenta $k_{F_i}$ of the intermediately propagating particle
\be
Q_F(k,\sqrt{s})=\Theta(k^2_1-k^2_{F_1})\Theta(k^2_2-k^2_{F_2})
\ee
and depends on $\sqrt{s}$ through the conserved total momentum, $P^2=s-(E_1+E_2)^2$, since
\be
\bm{k}_{1,2}=\pm \bm{k}+x_{1,2}\bm{P}
\ee
with the Lorentz-invariant transformation coefficients
\be
x_{1,2}=\frac{s\mp (m^2_2-m^2_1)}{2\sqrt{s}}
\ee
where the upper sign correlates with particle 1 and $x_1+x_2=1$. Thus, we find
\be
Q_F(k,P,u)=\Theta(k^2+x^2_1P^2+2x_1kPu-k_{F1})\Theta(k^2+x^2_1P^2-2x_1kPu-k_{F2})
\ee
where $u=cos(\beta)$ describes the angle between the vectors $\mathbf{k}$ and $\mathbf{P}$. In practice,  we use the angle-averaged projector
\be
\bar{Q}_F(k,P)=\frac{1}{2}\int^{+1}_{-1}{duQ_F(k,P,u)}
\ee
In nuclear matter, vector and scalar self-energies, $\Sigma^\mu=(\Sigma^0,\bm{k}E_i/M_i)^T$ and $\Sigma_s$, respectively, should be added, thius modifying the energies $E_i$ in the propagators Eq. \ref{eq:GBbS}. Thus, there are various sources of in-medium modifications. Among them, the Pauli-projector, however, provides typically the largest single contribution, as one easily sees from the Dyson-equation
\be
G^*=G-G\Sigma G^* \quad ,
\ee
relating the in-medium Green-function $G^*$ to the free-space propagator $G$. Hence, self-energy effects are suppressed by a factor $M$, $\Sigma/M \ll 1$. Similar conclusions will be found for self-energies contributions in in-medium spinors.

\begin{figure}[tbh]
\begin{center}
\includegraphics[width=8cm]{Fig04.eps}
\caption{In-medium Singlet-Even ($SE$) s-wave scattering lengths for the $S=-2$ double-hyperon channels as a function of the Fermi-momentum $k_F\sim \rho^{1/3}$ (see also \protect\cite{MD:2015}).}
\label{fig:Fig3}
\end{center}
\end{figure}

Results of our R-matrix calculations displayed below. As convenient measures for interactions we choose the low-energy parameters. For s-wave scattering at $q \to 0$ they are defined by
\be
\frac{1}{q}\tan{\delta_{s}(q,k_F)}\sim -a_{s}(k_F)\left(1+\frac{1}{2}q^2 a_{s}(k_F)r_{s}(k_F)+\cdots\right)
\ee
where $a_{s}$ and $r_{s}$ denote the scattering length and the effective range parameter, respectively. The scattering length is related to the volume integral of the R-matrix,  $a_{s}(k_F)=\frac{2\mu}{\hbar^2 4 \pi}R(0,k_F)_{|\ell=0}$, where $\mu$ is the reduced mass. Corresponding relations are found in all interaction channels. Thus, up to a normalization factor the scattering lengths correspond to in-medium effective coupling constants. As In Fig.(\ref{fig:Fig3}) the scattering lengths the singlet-even ($SE$) channels with vanishing total spin are displayed for the channels with strangeness $S=-2$. The interaction strength decreases rapidly in all channels with increasing density approaching a plateau at densities close to nuclear equilibrium. Overall, the scattering lengths are only about 10\% of the values found in the $NN$-system, for the latter see e.g. \cite{Machleidt:1989}, reflecting the much weaker $YY$ interaction.


With the T- and K-matrices available, we have access to the full scattering amplitude. For nuclear structure work we are interested in the first place on the G-matrix as introduced by Brueckner which is nothing than the in-medium K-matrix. While the natural representation of the K~-matrix is the \textit{singlet/triplet-even/odd} formalism, for nuclear matter calculations the explicit representation in terms of spin-isospin operators is more convenient. The two representation are related by an orthogonal transformation among the two operator sets. Thus, for each isospin doublet introduced in Eq.(\ref{eq:doublets}) we obtain in non-relativistic reduction a structure familiar from the nucleon sector,
\bea
R^{BB'}(\xi,k_F)&=&
\sum_{S,I=0,1}{R^{BB'}_{SI}(\xi,k_F)\left(\bm{\sigma}_B\cdot\bm{\sigma}_{B'}\right)^S\left(\bm{\tau}_B\cdot\bm{\tau}_{B'}\right)^I  } \nonumber \\ &+&\sum_{I=0,1}{\left(R^{BB'}_{TI}(\xi,k_F)\mathbf{S_{12}}+R^{BB'}_{LI}(\xi,k_F)\mathbf{L\cdot S}\right)\left(\bm{\tau}_B\cdot\bm{\tau}_{B'}\right)^I }
\eea
and also spin-orbit and rank-2 tensor terms are displayed. The amplitudes $R_{SI}(\xi,k_F)$ are given either in momentum space ($\xi={\mathbf{k_1,k_2}}$) or, if a static potential picture is an acceptable approximation, in coordinate space ($\xi={\mathbf{r_1,r_2}}$). For a given $(BB')$-combination some of the $R_{SI}$ may vanish. Formally, also the interactions involving the $\Sigma$~-isotriplet can be cast into such a form, except that one (or both) Pauli-type isospin operators have to be replaced by the proper spin-1 operator,  $\bm{\tau}_B\to \bm{T}_\Sigma$. In general, the $R_{SI}$ are functionals of the field operators, as studied in detail in our field-theoretical DDRH approach \cite{Fuchs:1995,Lenske:2004,Dejong:1998,Fedo:2014} and exploited later by many other groups by means of phenomenological mean-field parameterizations, e.g. \cite{lala}.  In a single-hyperon spin-saturated nucleus the hyperon mean-fields are then given by
\be
U^{YA}=U^{YA}_{0}+U^{YA}_{L0}\bm{\ell_Y}\cdot\bm{\sigma_Y}+\left(U^{YA}_{1}+U^{YA}_{L1}\bm{\ell_Y}\cdot\bm{\sigma_Y}\right) \tau^0_Y
\ee
where the central isoscalar and isovector potentials $U^{YA}_{0,1}(\rho_{0,1})$ are determined by the isoscalar and isovector nuclear densities, $\rho_{0,1}=\rho_n\pm\rho_p$, respectively. Similar expressions hold also for the spin-orbit terms. An open problem for the future is the consistent treatment of three- and many-body forces, urgently needed for neutron star physics, see e.g. \cite{Yama:2014}.


